Design for Hope: Cultivating Deliberate Hope in the Face of Complex Societal Challenges

Design has the potential to cultivate hope in the face of complex societal challenges. These challenges are often addressed through efforts aimed at harm reduction and prevention -- essential but sometimes limiting approaches that can unintentionally narrow our collective sense of what is possible. This one-day, in-person workshop builds on the first Positech Workshop at CSCW 2024 by offering practical ways to move beyond reactive problem-solving toward building capacity for proactive goal setting and generating pathways forward. We explore how collaborative and reflective design methodologies can help research communities navigate uncertainty, expand possibilities, and foster meaningful change. By connecting design thinking with hope theory, which frames hope as the interplay of ``goal-directed,'' ``pathways,'' and ``agentic'' thinking, we will examine how researchers might chart new directions in the face of complexity and constraint. Through hands-on activities including problem reframing, building a shared taxonomy of design methods that align with hope theory, and reflecting on what it means to sustain hopeful research trajectories, participants will develop strategies to embed a deliberately hopeful approach into their research.

==> inserts/diagram.tex <==
\begin{figure}[t]
    \centering
    \thispagestyle{empty}
    \includegraphics[width=0.6\linewidth]{file}
    \caption{caption}
    \Description {}
    \label{fig:}
\end{figure}


==> sections/3_agenda.tex <==
% \subsection{Workshop Themes and Goals}
% This workshop explores how design tools and processes can cultivate hope in research communities and society. Through structured activities, participants will explore problem reframing, examine design methods, and develop strategies for building hopeful research trajectories---both individually and collectively. 
% Detailed workshop themes are as follows:

% \begin{itemize}
%     \item \textbf{Reframing Challenges Through Design.} The way a designer frames a problem can affect the extent to view that problem with hope. This workshop will explore how design methods can break cognitive fixations, reframe challenges, and reveal new pathways forward. 
%     \item \textbf{Hope as a Process: Pathways and Agency in Research.} Hope is more than optimism---it requires concrete grounds and steps forward. Design aligns closely with the cognitive processes of hope. Participants will examine how design methods support hopeful thinking by fostering iteration, creativity, and strategic adaptation in research and practice.
%     \item \textbf{Building and Sustaining Hopeful Communities.} 
%     % Hope is not just an individual mindset---it is valuable at communal and societal levels, too. It is also strengthened through relationships, shared knowledge, and collective action.
%     This theme focuses on how researchers and stakeholders can create communities that reinforce hopeful thinking, sustain progress, and support each other in navigating challenges. We will examine strategies for fostering feedback loops, knowledge-sharing networks, and collaborative problem-solving.
%     % \item \textbf{Critical Thinking, Ethics, and Responsibilities of Hope in Design.} This workshop will also explore how speculative, participatory, and critical design approaches can anticipate unintended consequences and engage with complexity. Participants will reflect on how to balance visionary design with ethical considerations and societal impact.
%     \item \textbf{From Reflection to Action.} Beyond discussion, this workshop aims to generate tangible outcomes. Participants will contribute to a taxonomy of design methods aligned with hope, curate examples of design-driven hope in research, and establish a community space for continued engagement. The goal is not just to inspire but to equip participants with concrete strategies to integrate hopeful design into their research and beyond.
% \end{itemize}

% By organizing the workshop around these themes, we aim to provide participants with tools and perspectives that foster hope---both in the research they conduct and in the broader societal challenges they seek to address.

% \subsection{Anticipated Outcomes}
% This workshop will produce concrete resources and foster an ongoing community broadly centered on approaching research from an angle of hope. The key outcomes include:
% \begin{enumerate}
%     \item \textbf{Taxonomy of Design Methods and Their Relevance to Hope.} We will develop a taxonomy of design methods and their role in fostering hope. The taxonomy will cover dimensions such as but not limited to goal setting, pathways thinking, agentic thinking, and critical hope. It will also explore how existing methods can be refined to better support, for example, stakeholder engagement and researcher resilience.
%     % This taxonomy aims to provide researchers with a structured framework for reframing problems, identifying effective pathways toward goals, and incorporating communities meaningfully throughout the process, ultimately enabling more impactful and inclusive (human-centered and societal) research.
%     \item \textbf{Curated List of Design Work Showcasing Hope.} A collection of relevant design-related research (e.g., methods, design techniques, evaluation metrics) demonstrating how design fosters hope will be compiled and published. This will highlight projects that inspire us to envision and reimagine futures within complex and intractable problem spaces, showcasing hopeful design practices in action~\cite{kim2025socialmediaisntjust,somanath2022exploring,somanath2024design,radesky2022moral,hiniker2022reclaiming,yavo2024behind}.
%     \item \textbf{Online Community for Continued Engagement.} An online community space such as Discord or Slack for participants and other interested researchers to share insights, collaborate, and continue discussions beyond the workshop. This will serve as a hub for networking, resource-sharing, and sustained exploration of hopeful research.
% \end{enumerate}

% The taxonomy and the reading list will be made publicly available on our website for access and feedback.



\section{Workshop Activities}
The workshop will consist of a series of hands-on sessions and collaborative discussions. The full schedule can be found in Table~\ref{tab:schedule}.

\subsection*{Design as Hope: Introduction and Motivation}
\noindent Each participant introduces themselves, sharing what brought them to the workshop and their perspective on design as hope, including their definition of hope and how they see the design as hope framework being relevant to them.\\
\noindent > \textit{Format:} Full group sharing

\subsection*{[Activity 1] Problem Reframing: What Are We Really Hoping For?}
\noindent Participants will explore how problem reframing can unlock new pathways for action and impact. The activity consists of two parts:
\vspace{-1mm}
\begin{itemize}
    \item Part 1: Participants will discuss real-world cases where problem reframing led to breakthroughs, examining how different framings shaped hope and potential for action.
    \item Part 2: In small groups with shared interests, participants will select problems they are stakeholders of but have not researched as researchers. They will:
    \begin{itemize}
        \item Share and discuss their selected problems.
        \item Collaboratively reframe these problems, exploring alternative perspectives.
        \item Discuss how different framing influences their sense of hope and the specific actions and strategies they envision as part of the hopeful thinking process.
        \item Discuss helpful and (potential) challenging aspects of reframing techniques.
    \end{itemize}
\end{itemize}
\noindent > \textit{Format:} Small group discussion

\subsection*{[Activity 2] Taxonomy: Design Methods and Their Relevance to Hope}
\noindent In small groups, participants will select and analyze methods through:
\vspace{-1mm}
\begin{itemize}
    \item What were some success cases? Why would you consider them successful? What factors contributed to their success?
    \item What were some setbacks you experienced? What can we learn from these experiences?
    \item How can we make the best use of these methods to support pathways thinking?
    \item How can we improve stakeholder involvement in these methods?
    \item What's missing in aligning these methods with hope development? How might we address these gaps?
    \item How do these methods align with agentic thinking, what's missing, and how to better align them with hope?
\end{itemize}
\noindent > \textit{Format:} Small group discussion\\
\noindent > \textit{Pre-Workshop Preparation:} A comprehensive list of generative and iterative design methods will be provided as cards for discussion.

\subsection*{[Activity 3] Leveraging Communities: Designing Hopeful Future With Stakeholders and Fellow Researchers}
\noindent In small groups, participants will discuss two key themes on how to amplify the impact of design methods as instigators of hope.
\vspace{-1mm}
Knowledge-Sharing Focus:
\begin{itemize}
    \item How might we package this knowledge in ways helpful for other researchers or stakeholders?
    \item What are effective approaches for both short-term and long-term implementation?
    \item How might we create effective feedback loops for continuous improvement?
\end{itemize}
Community-Building Focus:
\begin{itemize}
    \item For both researchers and stakeholders, how might communities and relationships help with hope development?
    \item What approaches could make these communities better aligned with hope development?
    \item How might researchers impact/interact with stakeholder communities and vice versa?
    \item How can we make these crossover interactions more beneficial for all parties and societal hope?
\end{itemize}
\noindent > \textit{Format:} Small group discussion and then brief full group sharing

\subsection*{[Activity 4] Reflection: Designing Hopeful Research Trajectories for Self}
\noindent Participants personally reflect on the day's discussions and envision how they might approach their research differently to cultivate more hope---both for themselves as individuals in society, as researchers, and for their impact on society through research. 
\vspace{-1mm}
\begin{itemize}
    \item What might we want to do differently in our research practice?
    \item How has the workshop helped or not helped with hope development?
    \item What support would be helpful for achieving our goals or hopeful futures?
\end{itemize}
\noindent > \textit{Format:} Individual reflection with voluntary group sharing

\subsection*{Closing Reflections}
\noindent Reflect on the workshop's key takeaways and consider how to apply design as a tool for hope beyond the session.\\
\noindent > \textit{Format:} All group discussion

\begin{table}[!h]
    \centering
    \begin{tabular}{l p{6.2cm}}
        \hline
        \textbf{Time} & \textbf{Session} \\
        \hline
        9:00 - 9:15  & Welcome and Organizer Introduction \\
        9:15 - 9:45  & Introduction and Motivation \\
        9:45 - 10:30 & [Activity 1] Problem Reframing: What Are We Really Hoping For? \\
        10:30 - 11:00 & Coffee Break \\
        11:00 - 12:30 & [Activity 2] Taxonomy: Design Methods and Their Relevance to Hope \\
        12:30 - 2:00  & Lunch \\
        2:00 - 3:00   & [Activity 3] Leveraging Communities: Designing Hopeful Future With Stakeholders and Fellow Researchers \\
        3:00 - 3:30   & Coffee Break \\
        3:30 - 4:45   & [Activity 4] Reflection: Designing Hopeful Research Trajectories for Self \\
        4:45 - 5:00   & Closing Reflections \\
        \hline
    \end{tabular}
    \caption{Workshop Schedule}
    \label{tab:schedule}
\end{table}
